Syntactic structures and the general Markov models

We study phylogenetic signal present in syntactic information by considering the syntactic structures data from Longobardi (2017b), Collins (2010), Ceolin et al. (2020) and Koopman (2011). Focusing first on the general Markov models, we explore how well the the syntactic structures data conform to the hypothesis required by these models. We do this by comparing derived phylogenetic trees against trees agreed on by the linguistics community. We then interpret the methods of Ceolin et al. (2020) as an infinite sites evolutionary model and compare the consistency of the data with this alternative. The ideas and methods discussed in the present paper are more generally applicable than to the specific setting of syntactic structures, and can be used in other contexts, when analyzing consistency of data with against hypothesized evolutionary models.

==> influence_matrices/influence_k_1_nt.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  albanian &  greek &  hittite &  wt\_armenian \\
\midrule
01\_Subject Verb                                    &       0.0 &   15.5 &      4.5 &         16.5 \\
06\_Subject Object Verb                             &      13.0 &   17.5 &      5.5 &         17.5 \\
11\_Adposition Noun\_Phrase                          &       2.0 &   17.5 &      6.5 &         18.5 \\
12\_Noun\_Phrase Adposition                          &       3.0 &   19.5 &      7.5 &         19.5 \\
13\_Adjective Noun                                  &      16.0 &   19.5 &      8.5 &         20.5 \\
15\_Numeral Noun                                    &       5.0 &   20.5 &      9.5 &         21.5 \\
17\_Demonstrative Noun                              &       6.0 &   21.5 &     10.5 &         22.5 \\
19\_Possessor Noun                                  &      19.0 &   23.5 &     11.5 &         23.5 \\
21\_Pronominal Possessor Noun                       &      20.0 &   24.5 &     12.5 &         24.5 \\
A 01\_Attributive Adjective Agreement               &       9.0 &   24.5 &     13.5 &         24.5 \\
A 02\_Predicate Adjective Agreement                 &      10.0 &   25.5 &     14.5 &         25.5 \\
Neg 01\_Standard Negation is Particle that Prece... &      11.0 &   26.5 &     15.5 &         26.5 \\
Neg 03\_Standard Negation is Prefix                 &      24.0 &   28.5 &     18.5 &         28.5 \\
Neg 04\_Standard Negation is Suffix                 &      25.0 &   29.5 &     19.5 &         28.5 \\
Neg 07\_Standard Negation is Tone                   &      26.0 &   30.5 &     20.5 &         29.5 \\
Neg 08\_Standard Negation is Tone plus Other Mod... &      27.0 &   31.5 &     21.5 &         30.5 \\
Neg 09\_Standard Negation is Reduplication          &      28.0 &   32.5 &     22.5 &         31.5 \\
Neg 10\_Standard Negation is Infix                  &      29.0 &   33.5 &     23.5 &         32.5 \\
Neg 12\_Distinct Negation of identity               &      30.0 &   34.5 &     24.5 &         33.5 \\
Neg 13\_Distinct Negation of Existence              &      31.0 &   35.5 &     25.5 &         34.5 \\
Neg 14\_Distinct Negation of Location               &      32.0 &   36.5 &     26.5 &         35.5 \\
Order N3 01\_ Demonstrative Adjective Noun          &      21.0 &   36.5 &     25.5 &         37.5 \\
\bottomrule
\end{tabular}


==> influence_matrices/influence_k_2_nt.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  albanian &       greek &     hittite &  wt\_armenian \\
\midrule
01\_Subject Verb                                    &      26.0 &   86.166667 &   52.500000 &        209.0 \\
06\_Subject Object Verb                             &     127.0 &  107.500000 &   53.500000 &        210.0 \\
11\_Adposition Noun\_Phrase                          &      28.0 &   88.166667 &   54.500000 &        211.0 \\
12\_Noun\_Phrase Adposition                          &      29.0 &  109.500000 &   55.500000 &        212.0 \\
13\_Adjective Noun                                  &     130.0 &   90.166667 &   56.500000 &        213.0 \\
15\_Numeral Noun                                    &      31.0 &   91.166667 &   57.500000 &        214.0 \\
17\_Demonstrative Noun                              &      32.0 &   92.166667 &   58.500000 &        215.0 \\
19\_Possessor Noun                                  &     133.0 &  113.500000 &   59.500000 &        216.0 \\
21\_Pronominal Possessor Noun                       &     134.0 &  114.500000 &   60.500000 &        217.0 \\
A 01\_Attributive Adjective Agreement               &      35.0 &   95.166667 &   61.500000 &        217.0 \\
A 02\_Predicate Adjective Agreement                 &      36.0 &   96.166667 &   62.500000 &        218.0 \\
Neg 01\_Standard Negation is Particle that Prece... &      37.0 &   97.166667 &   63.500000 &        219.0 \\
Neg 03\_Standard Negation is Prefix                 &     138.0 &  118.500000 &  107.166667 &        221.0 \\
Neg 04\_Standard Negation is Suffix                 &     139.0 &  119.500000 &  108.166667 &        221.0 \\
Neg 07\_Standard Negation is Tone                   &     140.0 &  120.500000 &  109.166667 &        222.0 \\
Neg 08\_Standard Negation is Tone plus Other Mod... &     141.0 &  121.500000 &  110.166667 &        223.0 \\
Neg 09\_Standard Negation is Reduplication          &     142.0 &  122.500000 &  111.166667 &        224.0 \\
Neg 10\_Standard Negation is Infix                  &     143.0 &  123.500000 &  112.166667 &        225.0 \\
Neg 12\_Distinct Negation of identity               &     144.0 &  124.500000 &  113.166667 &        226.0 \\
Neg 13\_Distinct Negation of Existence              &     145.0 &  125.500000 &  114.166667 &        227.0 \\
Neg 14\_Distinct Negation of Location               &     146.0 &  126.500000 &  115.166667 &        228.0 \\
Order N3 01\_ Demonstrative Adjective Noun          &      47.0 &  107.166667 &   73.500000 &        230.0 \\
\bottomrule
\end{tabular}


==> influence_matrices/influence_k_3_nt.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &     albanian &        greek &     hittite &  wt\_armenian \\
\midrule
01\_Subject Verb                                    &  2255.066667 &  2386.733333 &   52.500000 &       1199.0 \\
06\_Subject Object Verb                             &  1793.800000 &  1922.800000 &   53.500000 &       1200.0 \\
11\_Adposition Noun\_Phrase                          &  2257.066667 &  2388.733333 &   54.500000 &       1201.0 \\
12\_Noun\_Phrase Adposition                          &  2258.066667 &  1924.800000 &   55.500000 &       1202.0 \\
13\_Adjective Noun                                  &  1796.800000 &  2390.733333 &   56.500000 &       1203.0 \\
15\_Numeral Noun                                    &  2260.066667 &  2391.733333 &   57.500000 &       1204.0 \\
17\_Demonstrative Noun                              &  2261.066667 &  2392.733333 &   58.500000 &       1205.0 \\
19\_Possessor Noun                                  &  1799.800000 &  1928.800000 &   59.500000 &       1206.0 \\
21\_Pronominal Possessor Noun                       &  1800.800000 &  1929.800000 &   60.500000 &       1207.0 \\
A 01\_Attributive Adjective Agreement               &  2264.066667 &  2395.733333 &   61.500000 &       1252.0 \\
A 02\_Predicate Adjective Agreement                 &  2265.066667 &  2396.733333 &   62.500000 &       1253.0 \\
Neg 01\_Standard Negation is Particle that Prece... &  2266.066667 &  2397.733333 &   63.500000 &       1254.0 \\
Neg 03\_Standard Negation is Prefix                 &  1804.800000 &  1933.800000 &  135.166667 &       1211.0 \\
Neg 04\_Standard Negation is Suffix                 &  1805.800000 &  1934.800000 &  136.166667 &       1256.0 \\
Neg 07\_Standard Negation is Tone                   &  1806.800000 &  1935.800000 &  137.166667 &       1257.0 \\
Neg 08\_Standard Negation is Tone plus Other Mod... &  1807.800000 &  1936.800000 &  138.166667 &       1258.0 \\
Neg 09\_Standard Negation is Reduplication          &  1808.800000 &  1937.800000 &  139.166667 &       1259.0 \\
Neg 10\_Standard Negation is Infix                  &  1809.800000 &  1938.800000 &  140.166667 &       1260.0 \\
Neg 12\_Distinct Negation of identity               &  1810.800000 &  1939.800000 &  141.166667 &       1261.0 \\
Neg 13\_Distinct Negation of Existence              &  1811.800000 &  1940.800000 &  142.166667 &       1262.0 \\
Neg 14\_Distinct Negation of Location               &  1812.800000 &  1941.800000 &  143.166667 &       1263.0 \\
Order N3 01\_ Demonstrative Adjective Noun          &  2276.066667 &  2407.733333 &   73.500000 &       1220.0 \\
\bottomrule
\end{tabular}


==> influence_matrices/influence_nt.tex <==
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
{} &  albanian/k=1 &  albanian/k=2 &  albanian/k=3 &  greek/k=1 &   greek/k=2 &    greek/k=3 &  hittite/k=1 &  hittite/k=2 &  hittite/k=3 &  western\_armenian/k=1 &  western\_armenian/k=2 &  western\_armenian/k=3 \\
\midrule
01\_Subject Verb                                    &           0.0 &          26.0 &   2255.066667 &       15.5 &   86.166667 &  2386.733333 &          4.5 &    52.500000 &    52.500000 &                  16.5 &                 209.0 &                1199.0 \\
06\_Subject Object Verb                             &          13.0 &         127.0 &   1793.800000 &       17.5 &  107.500000 &  1922.800000 &          5.5 &    53.500000 &    53.500000 &                  17.5 &                 210.0 &                1200.0 \\
11\_Adposition Noun\_Phrase                          &           2.0 &          28.0 &   2257.066667 &       17.5 &   88.166667 &  2388.733333 &          6.5 &    54.500000 &    54.500000 &                  18.5 &                 211.0 &                1201.0 \\
12\_Noun\_Phrase Adposition                          &           3.0 &          29.0 &   2258.066667 &       19.5 &  109.500000 &  1924.800000 &          7.5 &    55.500000 &    55.500000 &                  19.5 &                 212.0 &                1202.0 \\
13\_Adjective Noun                                  &          16.0 &         130.0 &   1796.800000 &       19.5 &   90.166667 &  2390.733333 &          8.5 &    56.500000 &    56.500000 &                  20.5 &                 213.0 &                1203.0 \\
15\_Numeral Noun                                    &           5.0 &          31.0 &   2260.066667 &       20.5 &   91.166667 &  2391.733333 &          9.5 &    57.500000 &    57.500000 &                  21.5 &                 214.0 &                1204.0 \\
17\_Demonstrative Noun                              &           6.0 &          32.0 &   2261.066667 &       21.5 &   92.166667 &  2392.733333 &         10.5 &    58.500000 &    58.500000 &                  22.5 &                 215.0 &                1205.0 \\
19\_Possessor Noun                                  &          19.0 &         133.0 &   1799.800000 &       23.5 &  113.500000 &  1928.800000 &         11.5 &    59.500000 &    59.500000 &                  23.5 &                 216.0 &                1206.0 \\
21\_Pronominal Possessor Noun                       &          20.0 &         134.0 &   1800.800000 &       24.5 &  114.500000 &  1929.800000 &         12.5 &    60.500000 &    60.500000 &                  24.5 &                 217.0 &                1207.0 \\
A 01\_Attributive Adjective Agreement               &           9.0 &          35.0 &   2264.066667 &       24.5 &   95.166667 &  2395.733333 &         13.5 &    61.500000 &    61.500000 &                  24.5 &                 217.0 &                1252.0 \\
A 02\_Predicate Adjective Agreement                 &          10.0 &          36.0 &   2265.066667 &       25.5 &   96.166667 &  2396.733333 &         14.5 &    62.500000 &    62.500000 &                  25.5 &                 218.0 &                1253.0 \\
Neg 01\_Standard Negation is Particle that Prece... &          11.0 &          37.0 &   2266.066667 &       26.5 &   97.166667 &  2397.733333 &         15.5 &    63.500000 &    63.500000 &                  26.5 &                 219.0 &                1254.0 \\
Neg 03\_Standard Negation is Prefix                 &          24.0 &         138.0 &   1804.800000 &       28.5 &  118.500000 &  1933.800000 &         18.5 &   107.166667 &   135.166667 &                  28.5 &                 221.0 &                1211.0 \\
Neg 04\_Standard Negation is Suffix                 &          25.0 &         139.0 &   1805.800000 &       29.5 &  119.500000 &  1934.800000 &         19.5 &   108.166667 &   136.166667 &                  28.5 &                 221.0 &                1256.0 \\
Neg 07\_Standard Negation is Tone                   &          26.0 &         140.0 &   1806.800000 &       30.5 &  120.500000 &  1935.800000 &         20.5 &   109.166667 &   137.166667 &                  29.5 &                 222.0 &                1257.0 \\
Neg 08\_Standard Negation is Tone plus Other Mod... &          27.0 &         141.0 &   1807.800000 &       31.5 &  121.500000 &  1936.800000 &         21.5 &   110.166667 &   138.166667 &                  30.5 &                 223.0 &                1258.0 \\
Neg 09\_Standard Negation is Reduplication          &          28.0 &         142.0 &   1808.800000 &       32.5 &  122.500000 &  1937.800000 &         22.5 &   111.166667 &   139.166667 &                  31.5 &                 224.0 &                1259.0 \\
Neg 10\_Standard Negation is Infix                  &          29.0 &         143.0 &   1809.800000 &       33.5 &  123.500000 &  1938.800000 &         23.5 &   112.166667 &   140.166667 &                  32.5 &                 225.0 &                1260.0 \\
Neg 12\_Distinct Negation of identity               &          30.0 &         144.0 &   1810.800000 &       34.5 &  124.500000 &  1939.800000 &         24.5 &   113.166667 &   141.166667 &                  33.5 &                 226.0 &                1261.0 \\
Neg 13\_Distinct Negation of Existence              &          31.0 &         145.0 &   1811.800000 &       35.5 &  125.500000 &  1940.800000 &         25.5 &   114.166667 &   142.166667 &                  34.5 &                 227.0 &                1262.0 \\
Neg 14\_Distinct Negation of Location               &          32.0 &         146.0 &   1812.800000 &       36.5 &  126.500000 &  1941.800000 &         26.5 &   115.166667 &   143.166667 &                  35.5 &                 228.0 &                1263.0 \\
Order N3 01\_ Demonstrative Adjective Noun          &          21.0 &          47.0 &   2276.066667 &       36.5 &  107.166667 &  2407.733333 &         25.5 &    73.500000 &    73.500000 &                  37.5 &                 230.0 &                1220.0 \\
\bottomrule
\end{tabular}

